Informal and Privatized Transit: Incentives, Efficiency and Coordination

Informal and privatized transit services, such as minibuses and shared auto-rickshaws, are integral to daily travel in large urban metropolises, providing affordable commutes where formal public transport is inadequate and other options are unaffordable. A defining feature of these systems is their decentralized, market-based organization, with drivers providing service in response to rider demand and earning opportunities. While this structure helps fill critical mobility gaps, it also generates inefficient service patterns when profit-driven driver route choices do not align with system-wide mobility goals. We develop an analytically tractable game-theoretic framework to study incentives underlying informal and privatized transit with a fixed menu of routes, quantify efficiency losses from decentralized driver route choice, and design incentive mechanisms to mitigate these inefficiencies. Here, profit-maximizing informal operators (drivers) decide where to provide service and cost-minimizing commuters (riders) decide whether to use these services. Within this framework, we establish a tight price of anarchy bound for cumulative driver profit and an instance-wise rider throughput bound whose dependence on per-rider profit heterogeneity is tight, showing that decentralized, profit-maximizing driver behavior can lead to substantial losses in cumulative driver profit and rider demand served. Moreover, we show that these losses can be mitigated through targeted interventions: budget-balanced cross-subsidization, which uses route-specific tolls/subsidies to shape driver payoffs, and fare optimization, which changes rider demand and driver margins through centrally regulated route-level fares. Finally, numerical experiments calibrated using data from an informal transit system in Nalasopara, India, reinforce these findings.

==> Fig/PoABounds/allocation_by_routes.tex <==
% Colors in matlab2tikz style
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.46600,0.67400,0.18800}%
\definecolor{mycolor4}{rgb}{0.49400,0.18400,0.55600}%

\begin{tikzpicture}

\begin{axis}[%
width=4.5in,
height=2.25in,
at={(0in,0in)},
scale only axis,
xmin=0,
xmax=2000,
ymin=0,
ymax=220,
xlabel style={font=\color{white!15!black}, font=\footnotesize, yshift=0.1cm},
xlabel={Cumulative Number of Drivers ($D$)},
ylabel style={font=\color{white!15!black}, font=\footnotesize},
ylabel={Drivers Allocated per Route},
ylabel style={yshift=-3pt},
%ytick={1.00,1.05,1.10,1.15, 1.20},
%yticklabels={1.00,1.05,1.10,1.15, 1.20},
%xtick={0.0,0.2,0.4,0.6, 0.8. 1.0},
%xticklabels={0.0, 0.0,0.2,0.4,0.6,0.8,1.0},
%title={OPT vs SR\_final: Profit Ratio across D},
title style={font=\footnotesize, yshift=-0.27cm},
tick label style={font=\scriptsize, yshift=0.07cm},
axis background/.style={fill=white},
grid=both,
grid style={dashed,gray!30},
legend style={
    at={(0.25,0.75)},
    anchor=east,
    legend cell align=left,
    align=left,
    draw=white!0!black,
    inner xsep=1pt,
    inner ysep=0pt,
    font=\tiny,
    row sep=-0.05cm
}
]

% Achole Gaon
\addplot[thick, mark=*, mark size=0.6pt]
coordinates {
(50,0.0) (100,0.0) (150,0.0) (200,0.0) (250,0.0)
(300,8.70025212994312) (350,19.7216414770899)
(400,28.5387529548073) (450,38.4580033672394)
(500,50.5815316491009) (550,54.8822914678434)
(600,56.6135940378069) (650,58.2678873700805)
(700,59.4255275165059) (750,60.8356247796095)
(800,62.5313913239888) (850,64.3244061289778)
(900,65.4982091605285) (950,66.7156479925085)
(1000,67.9792019317606) (1050,69.2915417373930)
(1100,71.5000370915729) (1150,73.5512676638721)
(1200,75.4055013024571) (1250,77.0236451072309)
(1300,78.0283013477600) (1350,79.0595123787876)
(1400,80.4776202241471) (1450,81.9475310958210)
(1500,83.0856912499296) (1550,85.0545464928189)
(1600,87.1189772329359) (1650,89.7325465499240)
(1700,92.5077799483752) (1750,94.9550757142053)
(1800,97.5353766847000) (1850,100.2598285474010)
(1900,103.1408581033610) (1950,105.5677018234400)
(2000,108.1115018673780)
};
\addlegendentry{Achole Gaon}

% Alkapuri
\addplot[thick, dashed, mark=square*, mark size=0.6pt]
coordinates {
(50,0.0) (100,0.0) (150,0.0)
(200,1.63662886803613) (250,14.9016480982466)
(300,25.5136634824149) (350,32.8501004998602)
(400,33.588305005475) (450,34.4594714177208)
(500,35.5876088748485) (550,36.5670843484682)
(600,37.7206201323316) (650,38.8228460452893)
(700,39.5941608673811) (750,40.5336833286410)
(800,41.6635420973836) (850,42.8581956342262)
(900,43.6402794961646) (950,44.4514371076175)
(1000,45.2933203861708) (1050,46.1677088106143)
(1100,47.6391895695183) (1150,49.0058876309389)
(1200,50.2413301762567) (1250,51.3194703087944)
(1300,51.9888547041265) (1350,52.6759320790709)
(1400,53.6207918473054) (1450,54.6001670408635)
(1500,55.3585026942088) (1550,56.6703155542611)
(1600,58.0458086502384) (1650,59.7871829097455)
(1700,61.6362710409747) (1750,63.2668602219529)
(1800,64.9860683801581) (1850,66.8013216868665)
(1900,68.7208998962592) (1950,70.3378622467594)
(2000,72.0327504936693)
};
\addlegendentry{Alkapuri}

% Ambawadi
\addplot[thick, dotted, mark=triangle*, mark size=0.6pt]
coordinates {
(50,0.0) (100,0.0) (150,0.0)
(200,0.0) (250,0.0) (300,0.0)
(350,0.0) (400,0.0) (450,0.0)
(500,0.0) (550,0.0) (600,0.0)
(650,0.0) (700,18.3700467057693)
(750,42.7535700200234)
(800,70.6204538077423)
(850,98.2751022217765)
(900,100.068443503196)
(950,101.92845174675)
(1000,103.858914848014)
(1050,105.863913204153)
(1100,109.238061832174)
(1150,112.371940655228)
(1200,115.204846722167)
(1250,117.677053733372)
(1300,119.211971825546)
(1350,120.787460439981)
(1400,122.954051658635)
(1450,125.199787761989)
(1500,126.938673703128)
(1550,129.94669914633)
(1600,133.100745242115)
(1650,137.093767599378)
(1700,141.333781030287)
(1750,145.072769946432)
(1800,149.014964781933)
(1850,153.177393965786)
(1900,157.579043217676)
(1950,161.286785411033)
(2000,165.173213975154)
};
\addlegendentry{Ambawadi}

% Evershine
\addplot[thick, dashdotted, mark=diamond*, mark size=0.6pt]
coordinates {
(50,0.0) (100,0.0) (150,0.0)
(200,0.0) (250,0.0)
(300,0.0) (350,0.0)
(400,13.8138795888977)
(450,29.6316788710115)
(500,48.9645446602617)
(550,64.7823439423755)
(600,82.3576764780574)
(650,98.1754757601712)
(700,108.72067528158)
(750,117.600089244332)
(800,120.878140512466)
(850,124.344180383792)
(900,126.613234770357)
(950,128.966640621107)
(1000,131.409190632871)
(1050,133.946047594895)
(1100,138.215244330987)
(1150,142.180435766713)
(1200,145.764816500327)
(1250,148.892816854411)
(1300,150.834897074252)
(1350,152.828309810916)
(1400,155.569624785102)
(1450,158.411079119077)
(1500,160.611232995731)
(1550,164.417186384255)
(1600,168.40789479164)
(1650,173.460131635389)
(1700,178.824877974628)
(1750,183.555694852264)
(1800,188.543621342814)
(1850,193.810202944569)
(1900,199.379461649873)
(1950,204.070743100458)
(2000,208.988110404083)
};
\addlegendentry{Evershine}

% Vijaynagar
\addplot[thick, loosely dotted, mark=o, mark size=0.6pt]
coordinates {
(50,0.0) (100,0.0) (150,0.0) (200,0.0)
(250,0.0) (300,0.0) (350,0.0) (400,0.0)
(450,0.0) (500,0.0) (550,0.0) (600,0.0)
(650,0.0) (700,0.0) (750,0.0) (800,0.0)
(850,0.0) (900,0.0) (950,0.0) (1000,0.0)
(1050,0.0) (1100,0.0) (1150,0.0) (1200,0.0)
(1250,7.41921398443397)
(1300,24.5477126639713)
(1350,41.6762113435086)
(1400,64.5142095828918)
(1450,87.3522078222748)
(1500,102.902275331705)
(1550,105.34071787511)
(1600,107.897531415768)
(1650,111.134457358241)
(1700,114.57160552396)
(1750,117.602600379091)
(1800,120.798323215479)
(1850,124.172578053901)
(1900,127.740755584185)
(1950,130.74642042146)
(2000,133.896936576194)
};
\addlegendentry{Vijaynagar}

% Firebrigade
\addplot[
    thick,
    densely dashed,
    mark=star,
    mark size=0.7pt
]
coordinates {
(50,0.0) (100,0.0) (150,0.0)
(200,17.3463802930434)
(250,27.7246777144680)
(300,36.0273156516077)
(350,46.4056130730323)
(400,54.7082510101720)
(450,60.0251777568831)
(500,61.9902877429716)
(550,63.6964424514937)
(600,65.7057939483863)
(650,67.6257684468781)
(700,68.9693267603922)
(750,70.6058870564015)
(800,72.5739954064057)
(850,74.6549701850841)
(900,76.0172871592644)
(950,77.4302478871318)
(1000,78.8967298546911)
(1050,80.4198327476388)
(1100,82.9830146678823)
(1150,85.3636749247477)
(1200,87.5157003430187)
(1250,89.3937196636843)
(1300,90.5597247027759)
(1350,91.7565492583192)
(1400,93.4024066441186)
(1450,95.1083866741482)
(1500,96.4293364890669)
(1550,98.7143918561064)
(1600,101.110372240963)
(1650,104.143683408192)
(1700,107.364622070301)
(1750,110.204955987505)
(1800,113.199655878470)
(1850,116.361657439321)
(1900,119.705383227807)
(1950,122.521980480226)
(2000,125.474317359268)
};
\addlegendentry{Firebrigade}

% Galanagar
\addplot[
    thick,
    loosely dotted,
    mark=triangle,
    mark size=0.7pt
]
coordinates {
(50,0.0) (100,0.0) (150,0.0) (200,0.0) (250,0.0)
(300,0.0) (350,0.0) (400,0.0) (450,0.0) (500,0.0)
(550,9.90979841843207)
(600,29.1858036014920)
(650,46.5342082662460)
(700,58.0998113760820)
(750,63.9518728461537)
(800,65.7345034481370)
(850,67.6193637620621)
(900,68.8532937577202)
(950,70.1330947569343)
(1000,71.4613730667247)
(1050,72.8409362533410)
(1100,75.1625597195830)
(1150,77.3188626623579)
(1200,79.2680776874594)
(1250,80.9691093974907)
(1300,82.0252282157188)
(1350,83.1092620687900)
(1400,84.6000111641943)
(1450,86.1452168475586)
(1500,87.3416781926636)
(1550,89.4113862067077)
(1600,91.5815654835696)
(1650,94.3290124480766)
(1700,97.2464045856460)
(1750,99.8190607916155)
(1800,102.531535269649)
(1850,105.395544634722)
(1900,108.424152239169)
(1950,110.975308762443)
(2000,113.649412588044)
};
\addlegendentry{Galanagar}


% Kargil
\addplot[
    thick,
    dashdotted,
    mark=diamond,
    mark size=0.7pt
]
coordinates {
(50,0.0) (100,0.0) (150,0.0) (200,0.0) (250,0.0)
(300,0.0) (350,0.0) (400,0.0) (450,0.0) (500,0.0)
(550,0.0) (600,0.0) (650,0.0) (700,0.0) (750,0.0)
(800,0.0)
(850,3.53593885642381)
(900,18.1480749228210)
(950,32.7602109892182)
(1000,47.3723470556154)
(1050,61.9844831220126)
(1100,85.3639008282480)
(1150,105.820891321204)
(1200,123.355454600881)
(1250,137.967590667278)
(1300,146.734872307116)
(1350,152.999776726511)
(1400,155.744167340439)
(1450,158.588809666292)
(1500,160.791432022768)
(1550,164.601655530417)
(1600,168.596841344262)
(1650,173.654746584589)
(1700,179.025511942876)
(1750,183.761636597449)
(1800,188.755159331076)
(1850,194.027649815184)
(1900,199.603156993781)
(1950,204.299701864223)
(2000,209.222586246493)
};
\addlegendentry{Kargil}

% Moregaon
\addplot[
    thick,
    loosely dashed,
    mark=pentagon*,
    mark size=0.7pt
]
coordinates {
(50,0.0) (100,0.0) (150,24.4130655536298)
(200,41.8521761238282)
(250,51.5405708850496)
(300,55.8480315813103)
(350,57.3823181632145)
(400,58.6718084590170)
(450,60.1935556524786)
(500,62.1641780101490)
(550,63.8751186893274)
(600,65.8901066605996)
(650,67.8154669201626)
(700,69.1627940775168)
(750,70.8039451234239)
(800,72.7775742557842)
(850,74.8643864208246)
(900,76.2305248591608)
(950,77.6474491130486)
(1000,79.1180447401896)
(1050,80.6454201212744)
(1100,83.2157920773309)
(1150,85.6031303746314)
(1200,87.7611924849162)
(1250,89.6444798772964)
(1300,90.8137557017829)
(1350,92.0139374951985)
(1400,93.6644117103590)
(1450,95.3751772210505)
(1500,96.6998324602318)
(1550,98.9912976844079)
(1600,101.393999084515)
(1650,104.435819057050)
(1700,107.665792842320)
(1750,110.514094240265)
(1800,113.517194627229)
(1850,116.688065985531)
(1900,120.041171329943)
(1950,122.865669478883)
(2000,125.826288020543)
};
\addlegendentry{Moregaon}


\end{axis}

% dummy axis (kept for matlab2tikz-style layout compatibility; can be removed)
\begin{axis}[%
width=0in,
height=0in,
at={(0in,0in)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left
]
\end{axis}

\end{tikzpicture}%

